Diffusion Prior-Based Amortized Variational Inference for Noisy Inverse Problems

Recent studies on inverse problems have proposed posterior samplers that leverage the pre-trained diffusion models as powerful priors. These attempts have paved the way for using diffusion models in a wide range of inverse problems. However, the existing methods entail computationally demanding iterative sampling procedures and optimize a separate solution for each measurement, which leads to limited scalability and lack of generalization capability across unseen samples. To address these limitations, we propose a novel approach, Diffusion prior-based Amortized Variational Inference (DAVI) that solves inverse problems with a diffusion prior from an amortized variational inference perspective. Specifically, instead of separate measurement-wise optimization, our amortized inference learns a function that directly maps measurements to the implicit posterior distributions of corresponding clean data, enabling a single-step posterior sampling even for unseen measurements. Extensive experiments on image restoration tasks, e.g., Gaussian deblur, 4$\times$ super-resolution, and box inpainting with two benchmark datasets, demonstrate our approach's superior performance over strong baselines. Code is available at https://github.com/mlvlab/DAVI.

==> Tables_supple/supple_imagenet.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Comparative results for noisy inverse problems (Colorization and motion deblurring on the ImageNet 256$\times$256}. The highest performance is highlighted in bold, while the second-highest one is underlined.}
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{l|c|ccccccc} 
\hline
       &             & \multicolumn{3}{c}{Colorization}                     &  & \multicolumn{3}{c}{Motion deblur}  \\
Method      & NFE $\downarrow$   & PSNR $\uparrow$ & LPIPS $\downarrow$ & FID $\downarrow$ &  & PSNR $\uparrow$ & LPIPS $\downarrow$ & FID $\downarrow$  \\ 
\hline
\hline
DDRM~\cite{kawar2022denoising}  & 20 &           22.26 & 0.243 & 47.17 &                     & - & - & - \\
DDNM$^+$\cite{wang2022zero}   & 100 &            21.38 & 0.310 & 78.13 &                     & - & - & - \\
DPS~\cite{chung2023diffusion} & 1000 &           17.67 & 0.578 & 93.25 &                     & 20.96 & 0.421 & 64.60 \\
$\Pi$GDM~\cite{song2023pseudoinverse}   & 100 &       20.58	& 0.276 & 54.01 &                & - & - & - \\
RED-diff~\cite{mardani2023variational} & 1000 &       22.51 & 0.353 & 66.72 &                & 22.45 & 0.456 & 88.73 \\
\hline
\textbf{DAVI (Ours)}  & 1 &            & & &                    & & & \\
\hline
\end{tabular}
}
\label{tab:supple_imagenet}
\end{table*}

